What Changed and What Could Have Changed? State-Change Counterfactuals for Procedure-Aware Video Representation Learning

Understanding a procedural activity requires modeling both how action steps transform the scene, and how evolving scene transformations can influence the sequence of action steps, even those that are accidental or erroneous. Existing work has studied procedure-aware video representations by modeling the temporal order of actions, but has not explicitly learned the state changes (scene transformations). In this work, we study procedure-aware video representation learning by incorporating state-change descriptions generated by Large Language Models (LLMs) as supervision signals for video encoders. Moreover, we generate state-change counterfactuals that simulate hypothesized failure outcomes, allowing models to learn by imagining unseen "What if" scenarios. This counterfactual reasoning facilitates the model's ability to understand the cause and effect of each step in an activity. We conduct extensive experiments on procedure-aware tasks, including temporal action segmentation, error detection, action phase classification, frame retrieval, multi-instance retrieval, and action recognition. Our results demonstrate the effectiveness of the proposed state-change descriptions and their counterfactuals, and achieve significant improvements on multiple tasks.

==> supp_sec/qualitative_results.tex <==
% \subsection{Full Results of Action Phase Classification \& Retrieval}
% \label{subsec:full}
% Tables \ref{table:ae2_cls} and \ref{table:ae2_retrieval} show classification and retrieval results on the Align-Ego-Exo~\cite{xue2023learning} dataset for each activity.

% \subsection{Qualitative Results}
% \label{sub}
% \begin{figure*}[t!]
% \centering
%         % \rule{0.8\textwidth}{5cm}
%         \includegraphics[width=17cm]{Figure/q1.pdf}
%         % \rule{0.8\textwidth}{5cm}
%         % \vspace{-1mm}
%         \caption{
%                  Qualitative results of Error Detection on EgoPER. GT denotes ground truth. \textcolor{OliveGreen}{Green}/\textcolor{red}{Red} segmentation and text denote the normal and error labels, respectively. The presented erroneous procedure \emph{``Make tea''} consists of [\emph{``\textcolor{red}{Not checking water temperature in the kettle},''} \emph{``\textcolor{OliveGreen}{{Hold the kettle,}}'' \emph{\textcolor{red}{``Pour water immediately,''} }\emph{\textcolor{red}{``Stir with the knife'',}} ....}].
%                  } 
        
%         \label{fig:qualitative}
%         \vspace{4mm}
% \end{figure*}


% \begin{figure*}[t!]
% \centering
%         % \rule{0.8\textwidth}{5cm}
%         \includegraphics[width=17cm]{Figure/q2.pdf}
%         % \rule{0.8\textwidth}{5cm}
%         % \vspace{-1mm}
%         \caption{
%                 Qualitative results of Temporal Action Segmentation on EgoPER. The example presents the procedure \emph{``Make Pinwheel''}. Distinct colored segments are different action step classes.
%                  } 
        
%         \label{fig:qualitative_2}
%         \vspace{3mm}
% \end{figure*}

% Figure~\ref{fig:qualitative} presents qualitative results on error detection in EgoPER, showing that our learned representations identify erroneous activities with greater fidelity. PVRL and HierVL produce several false positives, leading to over-segmentation, whereas our method better aligns with the ground-truth segments in both temporal location and count. 
% % 
% Figure~\ref{fig:qualitative_2} shows qualitative results on Temporal Action Segmentation, where PVRL and HierVL misclassify large temporal segments (dark and light orange, respectively). In contrast, our model more accurately distinguishes and classifies actions, reflecting an improved understanding of procedural activities and aligning with our quantitative results.

==> supp_sec/text_generation.tex <==
% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary


\section{Text Generation}
\label{sec:rationale}


\hank{generation details}


\hank{generation examples}
